Multiway Online Correlated Selection

We give a $0.5368$-competitive algorithm for edge-weighted online bipartite matching. Prior to our work, the best competitive ratio was $0.5086$ due to Fahrbach, Huang, Tao, and Zadimoghaddam (FOCS 2020). They achieved their breakthrough result by developing a subroutine called \emph{online correlated selection} (OCS) which takes as input a sequence of pairs and selects one item from each pair. Importantly, the selections the OCS makes are negatively correlated. We achieve our result by defining \emph{multiway} OCSes which receive arbitrarily many elements at each step, rather than just two. In addition to better competitive ratios, our formulation allows for a simpler reduction from edge-weighted online bipartite matching to OCSes. While Fahrbach et al. used a factor-revealing linear program to optimize the competitive ratio, our analysis directly connects the competitive ratio to the parameters of the multiway OCS. Finally, we show that the formulation of Farhbach et al. can achieve a competitive ratio of at most $0.5239$, confirming that multiway OCSes are strictly more powerful.

==> duplicatesOCS.tex <==
\section{Algorithm and analysis when the $A_j$ can contain duplicates}
\label{sec:duplicates}

In this section, we discuss how to modify our pseudocode in \Cref{fig:OCS meta algorithm} to handle the case where the $A_j$ passed to the OCS are multisets; i.e., allowed to contain multiple entries of the same element. The high level idea of our algorithm remains unchanged: Each vertex in $A_j$ is independently given a strength and the vertex with largest strength wins.

In order to determine the strength of $i \in A_j$, our algorithm reads the next $r$ entries of $i$'s strength distribution, where $r$ is the multiplicity of $i$ in $A_j$. Then, in order to determine the final strength of $i$ in this round, we apply the following two functions to those $r$ strengths.
\begin{enumerate}
    \item A win function, denoted $W_r$. This maps the $r$ separate strengths into a single desired win probability for $i$ in this round. We design these in \Cref{sec:win-functions}.
    \item A strength function, denoted $\BS_r$. This maps a desired win probability into a single strength for $i$ in this round. Importantly, $\BS_r$ is an increasing stochastic function with a continuous output. We design these in \Cref{sec:strength-functions}.
\end{enumerate}
The vertex with the largest combined strength (output of $\BS_r \circ W_r)$ wins the round. Since the output of $\BS_r$ is a continuous random variable, with probability $1$, their is a single vertex with maximal strength and we can ignore the possibly of a tie. We give pseudocode in \Cref{fig:OCS-generalized}.

\begin{figure}[h]
  \captionsetup{width=.9\linewidth}
\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt} 
$\mathrm{OCS}_{\mathcal{D}, W, \BS}$
\begin{enumerate}
    \item \textbf{Initialization:} For each $i \in L$, independently draw a strength sequence $\bx(i) \sim \mathcal{D}$ and initialize an index $k_i \leftarrow 1$
    \item Upon receiving $A_j = \{i_1, \ldots, i_m\}$
    \begin{enumerate}
        \item \textbf{Determine desired win probabilities:} or each $i \in A_j$, let $r_j(i)$ be the multiplicity of $i \in A_j$. Set the desired win probability of $i$ in this round to
        \begin{align*}
            \bw_j(i) = W_{r(i)}(\bx_{k_i}(i), \ldots, \bx_{k_i + r(i) - 1}(i))
        \end{align*}
        \item \textbf{Sample strengths:} For each $i \in A_j$, set the combined strength of $i$ in this round to
        \begin{align*}
            \bs_j(i) = \BS_{r(i)}(w_j(i))
        \end{align*}
        \item \textbf{Choose a winner:} Select the $i$ with maximal $\bs_j(i)$ among $i \in A_j$ as the winner.
        \item \textbf{Increment counters:} For each $i \in A_j$, increment $k_i \leftarrow k_i + r(i)$.
    \end{enumerate}
\end{enumerate}
\end{tcolorbox}
\caption{Our meta algorithm for constructing OCSs as a function of a strength distribution $\D$, win functions $W_1, \ldots, W_{m-1}$, and strength functions $\BS_1, \ldots, \BS_{m-1}$. This generalizes the pseudocode of \Cref{fig:OCS meta algorithm}}
\label{fig:OCS-generalized}
\end{figure}












\subsection{The win functions}
\label{sec:win-functions}
The goal of this subsection will be to design win functions $W_1, \ldots, W_{m-1}$ so that the following Lemma holds (note that the two criteria are exactly those of ($\diamondsuit$)).
\begin{lemma}
    \label{lem:win-functions-result}
    Let $W_1, \ldots, W_{m-1}$ be the functions defined \Cref{eq:def-Wr}. As long as the strength functions $\BS_1, \ldots, \BS_{m-1}$ satisfy
    \begin{enumerate}
        \item The strength functions are all stochastically increasing as in \Cref{def:stochastic-increasing}.
        \item In \Cref{fig:OCS-generalized}, the probability $i$ wins a round conditioned on $\bw_j(i) = w$ is at least $w$ for all $w \in [0,1]$.
    \end{enumerate}
    Then, the OCS in \Cref{fig:OCS-generalized} is an $(f,m)$-discrete OCS for the $f$ defined in \Cref{eq:f-from-all-strengths}.
\end{lemma}
In \Cref{sec:determining-icx}, we'll use \Cref{lem:icx-to-strength-dist,lem:large-diamond-holds} to show that the for our choice of $W_1, \ldots, W_{m-1}$, its possible to design strength functions satisfying the criteria in \Cref{lem:win-functions-result}.

How should we set $W_r$? Our goal is to satisfy,
\begin{align}
    \label{eq:desired-product}
    \Pr[i\text{ not selected in $n$ consecutive appearances}] \leq  \Ex_{\bx \sim \D}\left[\prod_{k = 1}^n \big(1 - W(\bx_k)\big)\right]
\end{align}
where $W$ is defined as in \Cref{lem:compute-w}. In the case of $r=1$, that task is easy: We set $W_1 = W$ and \Cref{lem:win-functions-result} follows from \Cref{lem:NA-implies-f}. As a first attempt, suppose we set
\begin{align}
    \label{eq:W-prod}
    W_r^{(\mathrm{prod})}(x_1, \ldots, x_r) \coloneqq 1 - \prod_{k = 1}^r \big(1 - W(\bx_k)\big)
\end{align}
It's not hard to see that with the above definition, \Cref{eq:desired-product} will hold. Unfortunately, the resulting $\bw^{(r)} = W_r^{(\mathrm{prod})}(\bx_1, \ldots, \bx_r)$ are not smaller, in the increasing convex order, than those of \Cref{lem:large-diamond-holds}. Therefore, we can't use our techniques to design strength functions satisfying the criteria of \Cref{lem:win-functions-result}. Instead, we'll set $W_r$ to an averaging of \Cref{eq:W-prod} over ``equivalent" inputs, for the following notion of equivalent.

\begin{definition}[$\D$-equivalent]
    \label{def:d-equiv}
    We say $(x_1, \ldots, x_r)$ and $(x_1', \ldots, x_r')$ are $\D$-equivalent, denoted
    \begin{align*}
        (x_1, \ldots, x_r) \Dequiv (x_1', \ldots, x_r')
    \end{align*}
    if for any index $k \geq 0$, the following distributions are equal.
    \begin{enumerate}
        \item The distribution of $\bx_1, \ldots, \bx_{k}, \bx_{k + r + 1}, \bx_{k + r + 2} \ldots$ where $\bx \sim \D$ conditioned on $\bx_{k +\ell} = x_\ell$ for $\ell = 1,\ldots, r$.
        \item The distribution of $\bx_1, \ldots, \bx_{k}, \bx_{k + r + 1}, \bx_{k + r + 2} \ldots$ where $\bx \sim \D$ conditioned on $\bx_{k +\ell} = x_\ell'$ for $\ell = 1,\ldots, r$.
    \end{enumerate}
    
\end{definition}
With the above definition in hand, we are able to define $W_r$:
\begin{align}
    \label{eq:def-Wr}
    W_r(x_1, \ldots, x_r) \coloneqq \Ex_{\bx \sim \D}\left[W_r^{(\mathrm{prod})}(\bx_1, \ldots, \bx_r) \mid (\bx_1, \ldots, \bx_r) \Dequiv (x_1, \ldots, x_r) \right]
\end{align}

\begin{proof}[Proof of \Cref{lem:win-functions-result}]
    For each $i \in L$ and $j \in [T]$, let $\bs_i^{(j)}$ be the value of $\bs_i$ in \Cref{fig:OCS-generalized} after receiving $A_j$. Then, as long as $\BS_1, \ldots, \BS_{m-1}$ are stochastically increasing, $\bs_i^{(1)},\bs_i^{(2)},\ldots$ are negatively associated. This follows from \Cref{prop:NA-closed-stochastically-increasing}, \Cref{lem:DN-NA}, and the fact that $W_r$ is an increasing function. Hence \Cref{lem:lose-disjoint-sets} holds, so we only need show the probability $i$ is never a winner in $n$ consecutive appearances is at most $f(n)$. Furthermore the following statement analogous to \Cref{lem:lose-seperate} holds: For any $i \in L$, subset of time steps $S \subseteq [T]$ in which $i$ appears, and desired win probabilities $w_j$ for each $j \in S$, 
    \begin{align}
        \label{eq:never-win}
        \Pr[i \text{ never a winner in } S \mid \bw_j(i) &= w_j \text{ for each } j \in S] \leq \prod_{j \in S} (1 - w_j).
    \end{align}
    
 
    Let $j_1, \ldots, j_m$ be consecutive time stamps in which $i$ appears, and $r_1, \ldots, r_m$ be its multiplicity in those time steps. We define $R_j \coloneqq \sum_{k=1}^j r_k$ and $n = R_m$. Then,
    \begin{align*}
        f(n) &= \Ex_{\bx \sim \D}\left[\prod_{k = 1}^n \big(1 - W(\bx_k)\big)\right] \tag{\Cref{eq:f-from-all-strengths}}\\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \prod_{\ell=1}^r \big(1 - W(\bx_{R_{j-1} + \ell})\big)\right]\tag{Expand product} \\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \Ex_{\bx' \sim \D} \left[\prod_{\ell=1}^r \big(1 - W(\bx'_{\ell})\big) \,\bigg|\, (\bx'_{1}, \ldots, \bx'_r) \Dequiv (\bx_{R_{j-1} + \ell}, \ldots, \bx_{R_j} \right] \right] \tag{\Cref{def:d-equiv}}\\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \bigg(1 - W_{r_j}(\bx_{R_{j-1} + 1}, \ldots, \bx_{R_{j}})  \bigg)\right] \tag{\Cref{eq:def-Wr}} \\
        & \geq \Pr\big[i \text{ never a winner in $n$ consecutive appearances}\big] \tag{\Cref{eq:never-win}}
    \end{align*}
    
\end{proof}

    


    
    
    















\subsection{Determining dominance in the increasing convex order}
\label{sec:determining-icx}
In this section, we will assert that it is possible to choose strength functions $\BS_1, \ldots, \BS_m$ meeting the criteria of \Cref{lem:win-functions-result}. As in \Cref{sec:strength-functions}, let $\bw^{(r)}$ be the output of $W_r(\bx_1, \ldots, \bx_r)$ for $\bx \sim \D$ and $W_r$ defined in \Cref{eq:def-Wr}. Let $\bv^{(1)}, \ldots, \bv^{(r)}$ be the corresponding random variables in \Cref{lem:large-diamond-holds}. Then, by \Cref{lem:icx-to-strength-dist}, it is enough for us to show that $\bw^{(r)} \icx \bv^{(r)}$ for all $r \in [m-1]$.

We'll use the following well known characterization.
\begin{fact}[\cite{SS07}]
    \label{fact:icx-expectations}
    For univariate random variables $\ba, \bb$, the following are equivalent.
    \begin{enumerate}
     \item $\ba$ is smaller than $\bb$ in the increasing convex order.
     \item For every $t \in \R$,
     \begin{align*}
         \Ex[(\ba - t)_+] \leq \Ex[(\bb - t)_+] .
     \end{align*}
     \end{enumerate}
\end{fact}

We use a mix of computational and analytical techniques to prove that $\bw^{(r)} \icx \bv^{(r)}$. In short, we do the following.
\begin{enumerate}
    \item First, we set an $x_{\max}$ and use $W^{\mathrm{(capped)}}$ in place of $W$, where
    \begin{align*}
        W^{\mathrm{(capped)}}(x) = W(\min(x, x_{\max}).
    \end{align*}
    Doing so slightly decreases the quality of our OCS but we set $x_{\max}$ large enough that this difference is rounding error. When computing the quality of our OCS using the dynamic programming procedure in \Cref{lem:compute-f-DP}, we use the same $W^{\mathrm{(capped)}}$, so the final competitive ratio we output will be a lower bound on what is truly achieved.
    \item When using $W^{\mathrm{(capped)}}$ in place of $W$, $\bw^{(r)}$ is a distribution with finite support. We compute the distribution. The function
    \begin{align*}
        t \mapsto \Ex[(\bw^{(r)}- t)_+]
    \end{align*}
    is piecewise linear in $t$, so we can store a complete description of it.
    \item We analytically compute the function:
    \begin{align*}
        t \mapsto \Ex[(\bv^{(r)}- t)_+].
    \end{align*}
    Using that, we are able to represent the function
    \begin{align*}
        t \mapsto \Ex[(\bv^{(r)}- t)_+] - \Ex[(\bw^{(r)}- t)_+].
    \end{align*}
    in a piecewise fashion. Given that piecewise representation, we just compute all extremal points -- those with derivative $0$ and the kinks -- and ensure the function is nonnegative at all such points. By \Cref{fact:icx-expectations}, this is sufficient.
\end{enumerate}





\newpage



\gray{
\pparagraph{The distribution $\BCC_r$:} We want the probability that $i \in A_j$ wins in round $j$ to be unaffected by the multiplicity of the other entries of $A_j$. $i$ wins round $j$ iff it has the maximal strength. Therefore, we want the following two distributions to be equal:
\begin{enumerate}
    \item The distribution of the max of $r$ independent copies of $\BCC_1(\bx)$ where $\bx$ is a single element from the strength distribution.
    \item The distribution of $\BCC_r(\bx_1, \ldots, \bx_r)$ where $\bx_1, \ldots, \bx_r$ are $r$ consecutive elements from the strength distribution.
\end{enumerate}
It's not hard to see (and we'll formally prove) that as long as $\BCC_r$ meets the above criteria, the probability that $i$ wins a round given its strength is unaffected by the multiplicity of other elements in $A_j$.

There are many equivalent ways to define the combination function. For any combination functions $\BCC_1, \ldots, \BCC_{m-1}$ and strictly increasing function $f:\R \to \R$, we could instead use $f \circ \BCC_1, \ldots, f \circ \BCC_{m-1}$ as our combination functions and the winners in every round would be identical. We'll ``normalize" our combination functions so that the following holds, which makes analysis more convenient.
\begin{align}
    \label{eq:win-equals-strength}
    \Pr[i \text{ wins a round in which it has strength }s] = s
\end{align}

Hence, we can think of the combination function as a ``requested win probability." Each vertex independently decides with what probability it should win the round using its strength distribution and the combination function. Then, the vertex with the highest requested win probability wins.

We begin by defining $\BCC_1$ a stochastic function mapping a single strength to a requested win probability. As in the proof of \Cref{lem:compute-w}, we can think of a single strength $\bx \sim \D^{(1)}$ as being generated in the following two step process:
\begin{align*}
    \text{Sample }\by \sim \Uniform(0,1) \quad\quad \text{then} \quad\quad \text{set }\bx = \min \{v \mid v\in \{-1, 0, 1, \ldots\}, G(v) \leq \by \}.
\end{align*}
To determine the combination function, we reverse this process. Given some $x$, we sample $\by \sim \Uniform(G(x), G(x + 1))$. As we proved in \Cref{lem:compute-w}, if we set the strength to this choice for $\by$, the probability $i$ wins given strength $x$ is $W(x)$. Therefore, the combination function mapping $x$ to $\Uniform(G(x), G(x + 1))$ gives the correct win probability. However, it doesn't satisfy \Cref{eq:win-equals-strength}. To remedy this, we apply a monotone transform $y \mapsto y^{m-1}$, setting
\begin{align}
    \label{eq:def-c1}
    \BCC_1(x) \coloneqq \by^{m-1} \quad \text{where} \quad \by \sim \Uniform(G(x), G(x + 1)).
\end{align}
For the above choice, \Cref{eq:win-equals-strength} is satisfied as we showed in the proof of \Cref{lem:compute-w}.

For $r \geq 2$, there is a natural choice for $\BCC_r$. We want the probability $i$ wins in a round in which it appears $r$ time to be the same as the probability it wins at least one of $r$ consecutive round in which it appears once. Therefore, a first attempt is to set,
\begin{align}
    \label{eq:combinations-first-attempt}
    \BCC_r(x_1, \ldots, x_r) = 1 - \prod_{k = 1}^r(1 - \BCC_1(x_k)).
\end{align}
Unfortunately the above choice for $\BCC_r$ won't work as it does not meet the earlier criteria that the output of $\BCC_r$ has the same distribution as the max of $r$ independent copies of $\BCC_1$. We introduce a general strategy for fixing this problem.

Let $\ba$ and $\bb$ be random variables coming from two distinct distributions. We want to ``adjust" $\ba$ so that it looks like it came from the same distribution as $\bb$. In our setting, $\ba$ is the output of \Cref{eq:combinations-first-attempt} where $\bx_1, \ldots, \bx_r \sim \D^{(r)}$, while $\bb$ is the max of $r$ independent copies of $\BCC_1(\bx)$ for $\bx \sim \D^{(1)}$. One way to do this is to define a coupling $(\ba, \bb)$ and then let the adjusted version of $\ba$ be drawn from
\begin{align*}
    \ba' \sim (\bb \mid \ba).
\end{align*}
Doing so will ensure that $\ba'$ has the same distribution of $\bb$. Depending on how the coupling is defined, we can try to guarantee that $\ba'$ is ``close to" $\ba$ for an appropriate definition of ``close to." In our context, we can think of $\ba$ as some desired win probability for a particular choice of strengths, and $\bb$ as drawn from some distribution of win probabilities we hope to match. If we use $\ba'$ in place of $\ba$, then by ensuring that $\Ex[\ba' \mid \ba] \geq \ba$, we can guarantee that a vertex wins with probability at least its desired win probability.

By \Cref{thm:mr01}, the existence of such a coupling is equivalent to the following notion of a stochastic ordering. For a thorough overview of stochastic orders, see \cite{SS07}.


We'll make use of the following powerful theorem of  M{\"u}ller and R{\"u}schendorf.
\begin{theorem}[\cite{MR01}]
    For univariate random variables $\ba, \bb$, the following are equivalent.
    \begin{enumerate}
        \item $\ba$ is smaller than $\bb$ in the increasing convex order.
        \item There is a coupling of $(\hat{\ba}, \hat{\bb})$ such that the marginal distribution of $\hat{\ba}$ and $\hat{\bb}$ are the same as those of $\ba$ and $\bb$ respectively, and, for any choice of $a$,
        \begin{align*}
            \Ex[\hat{\bb} \mid \hat{\ba}] \geq \hat{\ba}.
        \end{align*}
        Furthermore, the stochastic function mapping $a \mapsto (\hat{\bb} \mid \hat{\ba} = a)$ is increasing stochastically.
    \end{enumerate}
\end{theorem}
\Cref{thm:mr01} is a generalization of a classic result by Strassen \cite{s65} who proved the same result without the restriction that $a \mapsto (\hat{\bb} \mid \hat{\ba} = a)$ be increasing stochastically. We'll need the stronger result in our applications. With the above theorem in mind, we have the following plan of attack.
\begin{enumerate}
    \item Given strengths $x_1, \ldots, x_r$, decide on a desired win probability. We'll use $W_r$ to denote the deterministic function mapping $r$ strengths to a desired win probability (generalizing the $W$ in \Cref{lem:compute-w}). $W$ will be defined similarly to to the right hand side of \Cref{eq:combinations-first-attempt} but with adjustments so that the next step succeeds.
    \item Let $\ba$ the random variable indicating the output of $W_r$ on $\bx_1, \ldots, \bx_r \sim \Dr$. We also define $\bb$ to be the distribution of the max of $r$ independent copies of $\BCC_1(\bx)$ where $\bx \sim \D^{(1)}$. We prove that $\ba \icx \bb$ and then use \Cref{thm:mr01} to adjust $\ba$ so that the adjusted distribution is equal to the distribution of $\bb$ and $i$ still wins with the desired win probability. Then, we set $\BCC_r$ to be the adjusted $\ba$, where $\ba$ is the output of $W_r$.
\end{enumerate}


In order to execute the above plan of attack, we'll need to determine when $\ba \icx \bb$. We use the following well known characterization.
\begin{fact}[\cite{SS07}]
    For univariate random variables $\ba, \bb$, the following are equivalent.
    \begin{enumerate}
     \item $\ba$ is smaller than $\bb$ in the increasing convex order.
     \item For every $t \in \R$,
     \begin{align*}
         \Ex[(\ba - t)_+] \leq \Ex[(\bb - t)_+] .
     \end{align*}
     \end{enumerate}
\end{fact}

\subsection{Computing the desired win probability}

In this subsection, we'll define $W_r$, the function mapping $r$ strengths to a desired win probability. We set $W_1 = W$ where $W$ is defined as in \Cref{lem:compute-w}. Recall by \Cref{lem:NA-implies-f}, that if each $A_j$ contains only one copy of each vertex, then
\begin{align*}
    \Pr[i \text{ never selected in $n$ consecutive rounds}] \leq f(n) \coloneqq \Ex_{\bx \sim \D}\left[\prod_{k = 1}^n \big(1 - W_1(\bx_k)\big)\right]
\end{align*}
Now suppose $r > 1$. We wish to bound the probability that $r$ isn't selected in rounds $1, \ldots, m$ where the multiplicity of $i$ in $A_j$ is $r_j$. Our goal is for this probability to be at most $f(n)$ for $n = r_1 + \ldots + r_m$. Hence, our goal is to choose $W_r$ so that
\begin{align*}
    f\left(\sum_{j=1}^m r_j  \right) \overset{\mathrm{goal}}{=} \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \bigg(1 - W_{r_j}(\bx_{R_{j-1} + 1}, \ldots, \bx_{R_{j}})  \bigg)\right] \quad\quad \text{where } R_j \coloneqq \sum_{k=1}^j r_k
\end{align*}
In order to choose such a $W_r$, it will be helpful for us to determine when two settings for $x_1, \ldots, x_r$ are equivalent in the following sense.
\begin{definition}[$\D$-equivalent]
    We say $(x_1, \ldots, x_r)$ and $(x_1', \ldots, x_r')$ are $\D$-equivalent, denoted
    \begin{align*}
        (x_1, \ldots, x_r) \Dequiv (x_1', \ldots, x_r')
    \end{align*}
    if for any index $k \geq 1$, the following distributions are equal.
    \begin{enumerate}
        \item The distribution of $\bx_1, \ldots, \bx_{k}, \bx_{k + r + 1}, \bx_{k + r + 2} \ldots$ where $\bx \sim \D$ conditioned on $\bx_{k +\ell} = x_\ell$ for $\ell = 1,\ldots, r$.
        \item The distribution of $\bx_1, \ldots, \bx_{k}, \bx_{k + r + 1}, \bx_{k + r + 2} \ldots$ where $\bx \sim \D$ conditioned on $\bx_{k +\ell} = x_\ell'$ for $\ell = 1,\ldots, r$.
    \end{enumerate}
    
\end{definition}

Finally, we define $W_r$.
\begin{proposition}
    \label{prop:def-wr}
    For any $r \geq 1$, define
    \begin{align*}
        W_r(x_1, \ldots, x_r) \coloneqq \Ex_{\bx \sim \D}\left[1 - \prod_{k = 1}^r \big(1 - W_1(\bx_k)\big) \,\bigg|\, (\bx_1, \ldots, \bx_r) \Dequiv (x_1, \ldots, x_r) \right]
    \end{align*}
    Then, for any $m \geq 1$ and $r_1, \ldots, r_m \geq 0$
    \begin{align}
        \label{eq:W-effect}
        \Ex_{\bx \sim \D}\left[\prod_{k = 1}^{R_m}  \big(1 - W_1(\bx_k)\big)\right] = \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \bigg(1 - W_{r_j}(\bx_{R_{j-1} + 1}, \ldots, \bx_{R_{j}})  \bigg)\right] \quad\quad \text{where } R_j \coloneqq \sum_{k=1}^j r_k
    \end{align}
\end{proposition}
\begin{proof}
    The proof is a straightforward application of \Cref{def:d-equiv}, given below.
    \begin{align*}
        \Ex_{\bx \sim \D}&\left[\prod_{k = 1}^n \big(1 - W_1(\bx_k)\big)\right] \\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \prod_{\ell=1}^r \big(1 - W_1(\bx_{R_{j-1} + \ell})\big)\right] \\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \Ex_{\bx' \sim \D} \left[\prod_{\ell=1}^r \big(1 - W_1(\bx'_{\ell})\big) \,\bigg|\, (\bx'_{1}, \ldots, \bx'_r) \Dequiv (\bx_{R_{j-1} + \ell}, \ldots, \bx_{R_j} \right] \right] \\
        &= \Ex_{\bx \sim \D}\left[\prod_{j = 1}^m \bigg(1 - W_{r_j}(\bx_{R_{j-1} + 1}, \ldots, \bx_{R_{j}})  \bigg)\right].
    \end{align*}
\end{proof}


\subsection{Computing the desired distribution of win probabilities}

We determine the distribution of $\bb$, the max of $r$ independent copies of $\BCC_1(\bx)$ where $\bx \sim \D^{(1)}$.
\begin{lemma}
    \label{lem:desired-dist}
    For any $r \geq 1$, let $\bb_r$ the max of $r$ independent copies of $\BCC_1(\bx)$ where $\bx \sim \D^{(1)}$ and $\BCC_1$ is defined in \Cref{eq:def-c1}. For any $t \in [0,1]$
    \begin{align*}
        \Pr[\bb_r \leq t] = t^{\frac{r}{m-1}}.
    \end{align*}
\end{lemma}
\Cref{lem:desired-dist} is a special case of the following Lemma, which could be useful for other strength distributions.
\begin{lemma}
    \label{lem:desired-dist-general}
    For any $m,r \geq 1$, let $\mathcal{B}$ be a distribution supported on $[0,1]$ with the following properties.
    \begin{enumerate}
        \item The PDF of $\mathcal{B}$, $f_\mathcal{B}$ satisfies $f_{\mathcal{B}}(x) > 0$ for all $x \in [0,1]$.
        \item For $\bb^{(1)}, \ldots, \bb^{(m)}$ drawn independently from $\mathcal{B}$ and $b \in [0,1]$
        \begin{align*}
            \Pr[\bb^{(1)} \text{ is max of } (\bb^{(1)}, \ldots, \bb^{(m)}) \mid \bb^{(1)}  = b ] = b
        \end{align*}
    \end{enumerate}
    Then, for any $t \in [0,1]$,
    \begin{align*}
        \Prx_{\bb^{(1)}, \ldots, \bb^{(r)} \overset{\mathrm{iid}}{\sim} \mathcal{B}}[\max(\bb^{(1)}, \ldots, \bb^{(r)}) < t]  = t^{\frac{r}{m-1}}.
    \end{align*}
\end{lemma}
\begin{proof}
    Since $f_{\mathcal{B}}>0$, $\mathcal{B}$ has a strictly increasing CDF which we denote $F_{\mathcal{B}}$. We define,
    \begin{align*}
        \by^{(k)} = F_{\mathcal{B}}(\bb^{(k)})  \quad \quad \text{for }k = 1, \ldots, r.
    \end{align*}
    Since the CDF of $\mathcal{B}$ is strictly increasing, each $\by^{(k)}$ has a uniform distribution over $[0,1]$. We next solve for $F_{\mathcal{B}}$ using the second condition of \Cref{lem:desired-dist-general}
    \begin{align*}
        b &= \Pr[\bb^{(1)} \text{ is max of } (\bb^{(1)}, \ldots, \bb^{(m)}) \mid \bb^{(1)} = b] \\
        &= \prod_{k = 2}^m \Pr[\bb^{(k)} < b] \tag{Independence of $\bb^{(k)}$} \\
        &=  \prod_{k = 2}^m \Pr[\by^{(k)} < F_{\mathcal{B}}(b)] \tag{$  \by^{(k)} = F_{\mathcal{B}}(\bb^{(k)}) $} \\
        &=  ( F_{\mathcal{B}}(b))^{m-1} 
    \end{align*}
    So $F_{\mathcal{B}}(b) = b^{1/(m-1)}$. We compute the desired result.
    \begin{align*}
        \Prx[\max(\bb^{(1)}, \ldots, \bb^{(r)}) < t] &= \Prx[F^{-1}_{\mathcal{B}}(\max(\by^{(1)}, \ldots, \by^{(r)})) <t] \tag{$F_{\mathcal{B}}$ is strictly increasing} \\
        &=\Prx[\max(\by^{(1)}, \ldots, \by^{(r)}) <F_{\mathcal{B}}(t)] \\
        &=\prod_{k = 1}^r \Prx[\by^{(k)} <F_{\mathcal{B}}(t)] \tag{$\by^{(k)}$ are independent} \\
        &=\left(F_{\mathcal{B}}(t)\right)^{r} \tag{$\by^{(k)} \sim \Uniform(0,1)$} \\
        &=t^{r/(m-1)} \tag{$F_{\mathcal{B}}(b) = b^{1/(m-1)}$}
    \end{align*}
\end{proof}


\subsection{Determining dominance in the increasing stochastic order}
For each $r = 1, \ldots, m-1$, let $\ba_r = W_r(\bx_1, \ldots, \bx_r)$ where $\bx \sim \D$, and let $\bb_r$ be the max of $r$ independent copies of $\BCC_1(\bx)$ where $\bx \sim \D^{(1)}$. We use \Cref{fact:icx-expectations} to verify this holds. First, we compute $\E[(\bb_r - t)_+]$.
\begin{lemma}
    For any $t \in [0,1]$,
    \begin{align*}
        \E[(\bb_r - t)_+] = 1 - t - \frac{m-1}{r + m - 1} \cdot \left(1 - t^{\frac{r + m -1}{m - 1}}\right)
    \end{align*}
\end{lemma}
\begin{proof}
    This is a straightforward computation using \Cref{lem:desired-dist}.
    \begin{align*}
        \E[(\bb_r - t)_+] &= \int_{t}^{\infty} \Pr[\bb_r \geq x]dx \tag{integration by parts}\\
        &= \int_{t}^{1} \left(1 - x^{\frac{r}{m-1}} \right)dx \tag{$\bb_r \leq 1$ and \Cref{lem:desired-dist}} \\
        &= 1 - t - \frac{m-1}{r + m - 1} \cdot \left(1 - t^{\frac{r + m -1}{m - 1}}\right)
    \end{align*}
\end{proof}
Next we need to compute $\E[(\ba_r - t)_+]$ for each $t \in [0,1]$. This will be part computational and part analytic. We begin by giving a characterization of when two tuples are $\D$-equivalent that is easier to compute than that of \Cref{def:d-equiv}.

\begin{proposition}
    \label{prop:d-equiv-characterization}
    For any $x_1, \ldots, x_r$ and $x_1', \ldots, x_r'$ each containing at least one nonnegative element, if $z_{\mathrm{start}}(x_1, \ldots, x_r) = z_{\mathrm{start}}(x_1', \ldots, x_r')$ and $z_{\mathrm{end}}(x_1, \ldots, x_r) = z_{\mathrm{end}}(x_1', \ldots, x_r')$ then $(x_1, \ldots, x_r) \Dequiv (x_1', \ldots, x_r')$ where
    \begin{enumerate}
        \item $z_{\mathrm{start}}(v_1, \ldots, v_r)$ is defined, for $i_{\mathrm{first}}$ the smallest $i$ such that $v_i \geq 0$,
        \begin{align*}
            z_{\mathrm{start}}(x_1, \ldots, x_r) \coloneqq x_{i_{\mathrm{first}}} - i_{\mathrm{first}} + 1 
        \end{align*}
        \item $z_{\mathrm{end}}(v_1, \ldots, v_r)$ is defined, for $i_{\mathrm{last}}$ the largest $i$ such that $v_i \geq 0$,
        \begin{align*}
            z_{\mathrm{end}}(x_1, \ldots, x_r) \coloneqq r - i_{\mathrm{end}} 
        \end{align*}
    \end{enumerate}
\end{proposition}
\begin{proof}
    Fix any $k \geq 0$. For $\bx \sim \D$, our goal is to show the distribution of $(\bx_1, \ldots, \bx_k, \bx_{k + r + 1}, \ldots)$ is the same regardless of whether we condition on $\bx_{k + \ell} = x_\ell$ for all $\ell \in [r]$ or $\bx_{k + \ell} = x_\ell'$ for all $\ell \in [r]$. Let $\bz_{j}$ be the random variable indicating the state of $z$ in \Cref{fig:strength-unique} just before $\bx_j$ is generated.  Then, conditioning on $z_{\mathrm{start}}(\bx_{k + 1}, \ldots, \bx_{k + r}) = z_{k + 1}$ fixes $\bz_{k + 1} = z_{k + 1}$. Similarly, conditioning on $z_{\mathrm{end}}(\bx_{k + 1}, \ldots, \bx_{k + r}) = z_{k + r}$ fixes $\bz_{k + r} = z_{k + r}$. Therefore, regardless of whether we condition on $\bx_{k + \ell} = x_\ell$ for all $\ell \in [r]$ or $\bx_{k + \ell} = x_\ell$ for all $\ell \in [r]$, $\bz_{k + 1}$ and $\bz_{k + r}$ will be fixed to identical values. By \Cref{fact:memory-counter}, this implies that the distribution of $(\bx_1, \ldots, \bx_k, \bx_{k + r + 1}, \ldots)$ is the same regardless on which tuple we condition on.
\end{proof}
    
}


\newpage


\red{Still todo:}
\begin{enumerate}
    \item Give what the desired win probability will be as a function of the strengths $x_1, \ldots, x_r$.
    \item Show that $\ba \icx \bb$ for the above desired win probability (this step is computational)
    \item Discuss how one could implement this algorithm efficiently if they wanted to. Finding a coupling consistent with \Cref{thm:mr01} for discrete $\ba, \bb$ is a linear program. So, we can discretize $\ba, \bb$ to any desired accuracy and then run such a linear program.
\end{enumerate}


